The Explanation Game -- Rekindled (Extended Version)

Recent work demonstrated the existence of critical flaws in the current use of Shapley values in explainable AI (XAI), i.e. the so-called SHAP scores. These flaws are significant in that the scores provided to a human decision-maker can be misleading. Although these negative results might appear to indicate that Shapley values ought not be used in XAI, this paper argues otherwise. Concretely, this paper proposes a novel definition of SHAP scores that overcomes existing flaws. Furthermore, the paper outlines a practically efficient solution for the rigorous estimation of the novel SHAP scores. Preliminary experimental results confirm our claims, and further underscore the flaws of the current SHAP scores.

==> runex03.tex <==
\begin{figure}[t]
  \begin{subfigure}[b]{0.4325\linewidth} %\textwidth

    \begin{tabular}{c} ~~\\[5pt] \end{tabular}

    \centering
    \scalebox{0.875}{
      \renewcommand{\arraystretch}{1.15}
      \renewcommand{\tabcolsep}{0.575em}
      \input{./tabs/tr03}
    }
    %
    %\begin{tabular}{c} ~~\\[-2pt] \end{tabular}
    %
    \caption{Tabular representation (TR)}
  \end{subfigure}
  %
  \begin{subfigure}[b]{0.2585\linewidth} %\textwidth
    \centering
    \scalebox{0.85}{
      \input{./texfigs/dtex03}
    }
    \caption{Regression tree (RT)}
  \end{subfigure}
  %
  %
  \begin{subfigure}[b]{0.2775\linewidth} %\textwidth

    \begin{tabular}{c} ~~\\[5pt] \end{tabular}

    \centering
    \scalebox{0.875}{
      \renewcommand{\arraystretch}{1.15}
      \renewcommand{\tabcolsep}{0.575em}
      \input{./tabs/avg03}
    }

    \begin{tabular}{c} ~~\\[-1.0pt] \end{tabular}

    \caption{Expected values} \label{rex03:tab:avg}
  \end{subfigure}
  %
  \caption{Simple regression tree model, 
    adapted from~\cite[Fig.~8.1]{james-bk17}. 
    The target sample is $((1,1),1)$.}
  \label{fig:runex03}
\end{figure}


==> tabs/avg03.tex <==
\renewcommand{\tabcolsep}{0.45em}
\begin{tabular}{ccc} \toprule
  $\fml{S}$ & $\msf{rows}(\fml{S})$ & $\cfn{e}(\fml{S})$
  \\ \toprule
  $\emptyset$ & $1,2,3,4$ & $1-\alpha$ \\
  $\{x_1\}$ & $3,4$ & $1$ \\
  $\{x_2\}$ & $2,4$ & $1+\alpha$ \\
  $\{x_1,x_2\}$ & $4$ & $1$
  \\ \bottomrule
\end{tabular}


==> tabs/axpcxp01.tex <==
\begin{tabular}{cc} \toprule
  $\mbb{C}$ & $\{ \{1\}, \{2\} \}$ \\
  \midrule[0.75pt]
  $\mbb{A}$ & $\{ \{1,2\} \}$ \\
  \bottomrule
\end{tabular}


==> tabs/crit01.tex <==
\begin{tabular}{cc} \toprule
  WAXp & $\{i\in\fml{F}\,|\,\critic(i,\fml{S}\}$ \\
  \midrule[0.75pt]%\toprule
  $\{1,2\}$ & $\{1,2\}$ \\
  $\{1,2,3\}$ & $\{1,2\}$ \\
  $\{1,2,4\}$ & $\{1,2\}$ \\
  $\{1,2,3,4\}$ &  $\{1,2\}$ \\
  \bottomrule
\end{tabular}


==> tabs/crit01a.tex <==
% THIS IS NOT CORRECT; SEE NEW VERSION OF EXAMPLE
%
%\begin{tabular}{cc} \toprule
%  sbWAXps & $\{i\in\fml{F}\,|\,\critic(i,\fml{S}\}$ \\
%  \midrule[0.75pt]%\toprule
%  $\{1,2\}$ & $\{1,2\}$ \\
%  $\{1,2,3\}$ & $\{1,2\}$ \\
%  $\{1,2,4\}$ & $\{1,2\}$ \\
%  $\{1,2,3,4\}$ &  $\{1,2\}$ \\
%  \bottomrule
%\end{tabular}


==> tabs/sbaxp01.tex <==
\begin{tabular}{c} \toprule
  AXp \\
  \midrule[0.75pt]%\toprule
  $\{1,2\}$ \\
  \bottomrule
\end{tabular}


==> tabs/sbaxp01a.tex <==
\begin{tabular}{c|c} \toprule
  sbAXps & $\{\{1,2\}\}$ \\
  \bottomrule
\end{tabular}


==> tabs/sbcxp01.tex <==
\begin{tabular}{cccccc} \toprule
  $x_1$ & $x_2$ & $x_3$ & $x_4$ & {~} & set-based \\
  \midrule[0.75pt]%\toprule
  0 & 1 & 0 & 0 & & $\{2\}$ \\
  1 & 0 & 0 & 0 & & $\{1\}$\\
  \bottomrule
\end{tabular}


==> tabs/sbcxp01a.tex <==
\begin{tabular}{c|c} \toprule
  sbCXps & $\{ \{2\}, \{1\} \}$\\
  \bottomrule
\end{tabular}


==> tabs/sbwaxp01.tex <==
\begin{tabular}{c} \toprule
  WAXp\\
  \midrule[0.75pt]%\toprule
  $\{1,2\}$ \\
  $\{1,2,3\}$ \\
  $\{1,2,4\}$ \\
  $\{1,2,3,4\}$ \\
  \bottomrule
\end{tabular}


==> tabs/sbwaxp01a.tex <==
\begin{tabular}{c|c} \toprule
  sbWAXps & $\{\{1,2\},\{1,2,3\},\{1,2,4\},\{1,2,3,4\}\}$ \\
  \bottomrule
\end{tabular}


==> tabs/sbwcxp01.tex <==
\begin{tabular}{cccccc} \toprule
  $x_1$ & $x_2$ & $x_3$ & $x_4$ & {~} & set-based\\
  \midrule[0.75pt]%\toprule
  1 & 1 & 1 & 1 & & $\{1,2,3,4\}$ \\
  1 & 1 & 1 & 0 & & $\{1,2,3\}$ \\
  1 & 1 & 0 & 1 & & $\{1,2,4\}$ \\
  1 & 1 & 0 & 0 & & $\{1,2\}$ \\
  1 & 0 & 1 & 1 & & $\{1,3,4\}$ \\
  1 & 0 & 1 & 0 & & $\{1,3\}$ \\
  1 & 0 & 0 & 1 & & $\{1,4\}$ \\
  1 & 0 & 0 & 0 & & $\{1\}$ \\
  0 & 1 & 1 & 1 & & $\{2,3,4\}$ \\
  0 & 1 & 1 & 0 & & $\{2,3\}$ \\
  0 & 1 & 0 & 1 & & $\{2,4\}$ \\
  0 & 1 & 0 & 0 & & $\{2\}$ \\
  \bottomrule
\end{tabular}


==> tabs/sbwcxp01a.tex <==
\begin{tabular}{c|c} \toprule
  sbWCXps &
  $\{\{1\},\{2\},\{1,2\},\{1,3\},\{1,4\},\{2,3\},\{2,4\},\{1,2,3\},\{1,2,4\},\{1,3,4\},\{2,3,4\},\{1,2,3,4\}\}$ \\
  \bottomrule
\end{tabular}


==> tabs/sbwcxp01b.tex <==
\begin{tabular}{ccccccc} \toprule
  $1$ & $2$ & $3$ & $4$ & {~} &
  set-based, $\fml{S}$ &
  $\{i\,|\,\critic(i,\fml{S})\}$ \\
  \midrule[0.75pt]%\toprule
  1 & 1 & 1 & 1 & & $\{1,2,3,4\}$ & $\emptyset$ \\
  1 & 1 & 1 & 0 & & $\{1,2,3\}$ & $\emptyset$ \\
  1 & 1 & 0 & 1 & & $\{1,2,4\}$ & $\emptyset$ \\
  1 & 1 & 0 & 0 & & $\{1,2\}$ & $\emptyset$ \\
  1 & 0 & 1 & 1 & & $\{1,3,4\}$ & $\{1\}$ \\
  1 & 0 & 1 & 0 & & $\{1,3\}$ & $\{1\}$ \\
  1 & 0 & 0 & 1 & & $\{1,4\}$ & $\{1\}$ \\
  1 & 0 & 0 & 0 & & $\{1\}$ & $\emptyset$ \\
  0 & 1 & 1 & 1 & & $\{2,3,4\}$ & $\{2\}$ \\
  0 & 1 & 1 & 0 & & $\{2,3\}$ & $\{2\}$ \\
  0 & 1 & 0 & 1 & & $\{2,4\}$ & $\{2\}$ \\
  0 & 1 & 0 & 0 & & $\{2\}$ & $\emptyset$ \\
  \bottomrule
\end{tabular}


==> tabs/tab-res-bf.tex <==
\begin{tabular}{ccccccc} \toprule
  \multirow{2}{*}{Issue} &
  \multirow{2}{*}{Definition} &
  \multicolumn{5}{c}{$\epsilon$} \\ %error
  \Cline{0.75pt}{3-7}
  & & 0.1 & 0.05 & 0.01 & 0.005 & 0.001 \\
  \toprule%\midrule[0.75pt]
  I1 & $[\irrelevant(i)\land(\sv(i)\not=0)]$ & \\
  %
  I2 & $[\irrelevant(i_1)\land\relevant(i_2)\land(|\sv(i_1)|>|\sv(i_2)|)]$ & \\
  %
  I3 & $[\relevant(i)\land(\sv(i)=0)]$ &\\
  %
  I4 &
  $[\irrelevant(i_1)\land(\sv(i_1)\not=0)]\land[\relevant(i_2)\land(\sv(i_2)=0)]$
  & \\
  %
  I5 &
  $[\irrelevant(i)\land\forall(1\le{j}\le{m},j\not=u).(|\sv(j)|<|\sv(i)|)]$
  & \\ 
  %
  I6 &
  $[\irrelevant(i_1)\land\relevant(i_2)\land(\sv(i_1)\times\sv(i_2)>0)]$
  & \\
  %
  I7 &
  $[\irrelevant(i_1)\land\relevant(i_2)\land(|\sv(i_1)|>|\sv(i_2)|)\land(\sv(i_1)\times\sv(i_2)>0)]$
  & \\
  %
  I8 &
  $\forall(j\in\fml{F}).\left([\relevant(j)\land(\sv(j)=0)]\lor[\irrelevant(j)\land(\sv(j)\not=0)]\right)$
  & \\
  %
  I8 &
  $\forall(j\in\fml{F}).\left([\relevant(j)\land(\sv(j)=0)]\lor[\irrelevant(j)\land(\sv(j)\not=0)]\right)$
  & \\
  %
  I9 &
  $\exists(i\in\fml{F}).[\rnk{a}(i)\not=\rnk{e}(i)]$
  & \\
  \bottomrule
\end{tabular}


==> tabs/tr03.tex <==
\renewcommand{\tabcolsep}{0.45em}
\begin{tabular}{cccccc} \toprule
  row & $x_1$ & $x_2$ & $\rho(\mbf{x})$ &
  \makecell{$\rho_a(\mbf{x})$\\$\alpha=\sfrac{1}{2}$} &
  \makecell{$\rho_b(\mbf{x})$\\$\alpha=\sfrac{1}{4}$}
  \\ \toprule
  1 & 0 & 0 & $1-6\alpha$ & $-2$ & $-\sfrac{1}{2}$ \\
  2 & 0 & 1 & $1+2\alpha$ & $2$ & $\sfrac{3}{2}$ \\
  3 & 1 & 0 & 1           & 1               & 1 \\
  \tikzmarknode{a}{4} & 1 & 1 & 1           & 1               & \tikzmarknode{b}{1}
  \\ \bottomrule
  \begin{tikzpicture}[overlay,remember picture]
    \node[draw=midblue, thin, xshift=-0.35pt, yshift=-0.35pt, inner
      sep=2.0pt, fit=(a) (b)] {};
  \end{tikzpicture}
\end{tabular}


==> texfigs/dtex02.tex <==
% Concocted example
%%
%\tikzset{every label/.style={xshift=-0.35ex,
%  yshift=-5.25ex,
%  text width=1ex,
%  align=right, inner sep=1pt, font=\tiny, text=midblue}}
%%
%\tikzset{tlabel/.style={xshift=0.25ex, yshift=1.75ex, text width=1ex,
%    align=right, inner sep=1pt, font=\tiny, text=midblue}}
%%%\tikzset{every node/.style={---rectangle---}}
%
\forestset{
  BDT/.style={
    for tree={
      l=1.5cm,s sep=1.15cm,
      if n children=0{}{circle}, %rectangle
      %if n children=0{}{draw},
      draw=midblue,%draw=black,%
      text=midblue,%text=black,%
      edge={
        my edge
      },
      %if n=1{
      %  edge+={0 my edge},
      %}{},
      edge=thick,
      %font=\sffamily,
    }
  },
}
%
\begin{forest}
  BDT
  [{$x_1$}, label={[yshift=-6.875ex]{{\tiny1}}} 
    [{$x_2$}, label={[yshift=-6.875ex]{{\tiny2}}}, %xshift=-3.075ex,yshift=-3.5ex
      edge label={node[midway,left,xshift=-1.5pt] {{\scriptsize$\in\{0\}$}}}
      [\ncolor{\boldmath{$1-6\alpha$}}, label={[yshift=-5.25ex]{{\tiny4}}},
        edge label={node[midway,left,xshift=-0.5pt]
          {{\scriptsize$\in\{0\}$}}}, rectangle, fill={torange1!10} ]
      [\ncolor{\boldmath{$1+2\alpha$}}, label={[yshift=-5.25ex]{{\tiny5}}},
        edge label={node[midway,right,xshift=-0.575pt] {{\scriptsize$\in\{1\}$}}}, rectangle, fill={torange1!10} ]
    ]
    [\ncolor{\textbf{1}}, label={[yshift=-5.25ex]{{\tiny3}}},
      edge={very thick,draw=tblue2}, edge label={node[midway,right,xshift=0.5pt] {{\scriptsize$\in\{1\}$}}},
      rectangle, fill={torange1!10} ]
  ]
\end{forest}


==> texfigs/dtex03.tex <==
\forestset{
  BDT/.style={
    for tree={
      l=1.5cm,s sep=1.15cm,
      if n children=0{}{circle}, %rectangle
      %if n children=0{}{draw},
      draw=midblue,%draw=black,%
      text=midblue,%text=black,%
      edge={
        my edge
      },
      %if n=1{
      %  edge+={0 my edge},
      %}{},
      edge=thick,
      %font=\sffamily,
    }
  },
}
%
\begin{forest}
  BDT
  [{$x_1$}, label={[xshift=-3ex,yshift=-3.7125ex]{{\tiny1}}} 
    [{$x_3$}, label={[yshift=-6.875ex]{{\tiny2}}}, %edge={very thick}, %top-left=x
      edge label={node[midway,left,xshift=-0.75pt] {{\scriptsize$\in\{0\}$}}}
      [\dghlight{\textbf{0}}, label={[yshift=-5.25ex]{{\tiny5}}},
        edge label={node[midway,left,xshift=-0.5pt] {{\scriptsize$\in\{0\}$}}},
        rectangle, fill={tblue2!25} ]
      [\dghlight{\textbf{1}}, label={[yshift=-5.25ex]{{\tiny6}}},
        edge label={node[midway,right,xshift=-0.5pt] {{\scriptsize$\in\{1\}$}}},
        rectangle, fill={tblue2!25} ]
    ]
    %
    [\dghlight{\textbf{1}}, label={[yshift=-5.25ex]{{\tiny3}}},
     edge label={node[near end,right,xshift=0.5pt] {{\scriptsize$\in\{1\}$}}},
      rectangle, fill={tblue2!25} ]
    %
    [{$x_4$}, label={[yshift=-6.875ex]{{\tiny4}}}, %edge={very thick}, %top-left=x
       edge={very thick,draw=purple3}, edge label={node[midway,right,xshift=0.25pt] {{\scriptsize$\in\{2\}$}}}
      [\dghlight{\textbf{1}}, label={[yshift=-5.25ex]{{\tiny7}}},
        edge label={node[midway,left,xshift=-0.5pt] {{\scriptsize$\in\{0\}$}}},
        rectangle, fill={tblue2!25} ]
      [\dghlight{\textbf{0}}, label={[yshift=-5.25ex]{{\tiny8}}},
         edge={very thick,draw=purple3}, edge label={node[midway,right,xshift=-0.5pt] {{\scriptsize$\in\{1\}$}}},
        rectangle, fill={tblue2!25} ]
    ]
    %
  ]
\end{forest}

